Differentially Private Data-Driven Markov Chain Modeling

Markov chains model a wide range of user behaviors. However, generating accurate Markov chain models requires substantial user data, and sharing these models without privacy protections may reveal sensitive information about the underlying user data. We introduce a method for protecting user data used to formulate a Markov chain model. First, we develop a method for privatizing database queries whose outputs are elements of the unit simplex, and we prove that this method is differentially private. We quantify its accuracy by bounding the expected KL divergence between private and non-private queries. We extend this method to privatize stochastic matrices whose rows are each a simplex-valued query of a database, which includes data-driven Markov chain models. To assess their accuracy, we analytically bound the change in the stationary distribution and the change in the convergence rate between a non-private Markov chain model and its private form. Simulations show that under a typical privacy implementation, our method yields less than 2% error in the stationary distribution, indicating that our approach to private modeling faithfully captures the behavior of the systems we study.

==> Figures/eps_vs_peps_Tran.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{chocolate2267451}{RGB}{226,74,51}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue52138189}{RGB}{52,138,189}
\definecolor{black}{RGB}{0, 0, 0}
\definecolor{GTblue}{RGB}{0, 48, 87}
\definecolor{GTgold}{RGB}{179, 163, 105}
\definecolor{UFOrange}{RGB}{250, 70, 22}
\definecolor{UFblue}{RGB}{0, 33, 165}
%
\begin{tikzpicture}

\begin{axis}[%
width=0.35\figW,
height=0.56\figH,
axis background/.style={fill=gainsboro229},
axis line style={white},
%at={(0.758in,0.481in)},
scale only axis,
xlabel=\textcolor{black}{{Dirichlet Parameter,~$k$}},
xtick style={color=dimgray85},
x grid style={white},
yminorticks=true,
y grid style={white},
ylabel=\textcolor{black}{Privacy Strength, $\epsilon$},
xmajorgrids,
ymajorgrids,
yminorgrids,
tick align=outside,
tick pos=left,
%yticklabel={$\pgfmathprintnumber{\tick}$\%},
legend pos = north west,
legend style={nodes={scale=0.85, transform shape}},
% xmin=,
% xmax=10.5,
% ymin=-0.2,
% ymax=6.3,
]
\addplot [color=UFblue, ultra thick]
  table[row sep=crcr]{%
13.1578947368421	7.08400219162691\\
13.8157894736842	7.13881644845661\\
14.4736842105263	7.21612646748547\\
15.1315789473684	7.31094127025065\\
15.7894736842105	7.41966981226616\\
16.4473684210526	7.53966165878097\\
17.1052631578947	7.66891741794025\\
17.7631578947368	7.80589996964407\\
18.4210526315789	7.94940779492333\\
19.0789473684211	8.09848780764104\\
19.7368421052632	8.25237402522711\\
20.3947368421053	8.41044356242471\\
21.0526315789474	8.57218449568632\\
21.7105263157895	8.7371720228367\\
22.3684210526316	8.90505052261941\\
23.0263157894737	9.0755198779582\\
23.6842105263158	9.24832492557486\\
24.3421052631579	9.42324722861478\\
25	9.60009859649681\\
25.6578947368421	9.77871593373012\\
26.3157894736842	9.95895711008669\\
26.9736842105263	10.1406976232897\\
27.6315789473684	10.3238278821611\\
28.2894736842105	10.5082509795816\\
28.9473684210526	10.6938808551414\\
29.6052631578947	10.880640770089\\
30.2631578947368	11.0684620342714\\
30.9210526315789	11.2572829377136\\
31.5789473684211	11.4470478493921\\
32.2368421052632	11.6377064533929\\
32.8947368421053	11.8292130985672\\
33.5526315789474	12.0215262424368\\
34.2105263157895	12.2146079737414\\
34.8684210526316	12.4084236009115\\
35.5263157894737	12.6029412960474\\
36.1842105263158	12.7981317858285\\
36.8421052631579	12.9939680822583\\
37.5	13.190425247356\\
38.1578947368421	13.3874801868761\\
38.8157894736842	13.5851114689413\\
39.4736842105263	13.7832991641253\\
40.1315789473684	13.9820247040646\\
40.7894736842105	14.1812707561252\\
41.4473684210526	14.3810211120193\\
42.1052631578947	14.581260588581\\
42.7631578947368	14.781974939165\\
43.421052631579	14.9831507743542\\
44.0789473684211	15.1847754908429\\
44.7368421052632	15.386837207519\\
45.3947368421053	15.5893247078988\\
46.0526315789474	15.7922273881832\\
46.7105263157895	15.9955352102956\\
47.3684210526316	16.1992386593458\\
48.0263157894737	16.4033287050357\\
48.6842105263158	16.6077967665788\\
49.3421052631579	16.812634680762\\
50	17.0178346728199\\
50.6578947368421	17.2233893298326\\
51.3157894736842	17.4292915763912\\
51.9736842105263	17.6355346523035\\
52.6315789473684	17.8421120921411\\
53.2894736842105	18.0490177064477\\
53.9473684210526	18.2562455644508\\
54.6052631578947	18.4637899781356\\
55.2631578947368	18.6716454875535\\
55.921052631579	18.8798068472544\\
56.5789473684211	19.0882690137391\\
57.2368421052632	19.2970271338428\\
57.8947368421053	19.506076533967\\
58.5526315789474	19.7154127100877\\
59.2105263157895	19.9250313184718\\
59.8684210526316	20.1349281670435\\
60.5263157894737	20.3450992073464\\
61.1842105263158	20.5555405270521\\
61.8421052631579	20.766248342971\\
62.5	20.9772189945257\\
63.1578947368421	21.1884489376501\\
63.8157894736842	21.3999347390807\\
64.4736842105263	21.6116730710114\\
65.1315789473684	21.8236607060815\\
65.7894736842105	22.035894512675\\
};
\addlegendentry{Theorem~\ref{thm:dp}}


\addplot [color=UFOrange, ultra thick]
  table[row sep=crcr]{%
13.1578947368421	2.40427397354128\\
13.8157894736842	2.52135312367871\\
14.4736842105263	2.63845032890192\\
15.1315789473684	2.75556336695326\\
15.7894736842105	2.87269036272044\\
16.4473684210526	2.98982972347634\\
17.1052631578947	3.10698008801237\\
17.7631578947368	3.22414028632371\\
18.4210526315789	3.34130930738986\\
19.0789473684211	3.45848627322288\\
19.7368421052632	3.57567041781289\\
20.3947368421053	3.69286106992934\\
21.0526315789474	3.81005763898235\\
21.7105263157895	3.92725960332982\\
22.3684210526316	4.04446650055228\\
23.0263157894737	4.1616779193221\\
23.6842105263158	4.27889349256984\\
24.3421052631579	4.39611289171462\\
25	4.51333582177107\\
25.6578947368421	4.63056201718013\\
26.3157894736842	4.74779123824496\\
26.9736842105263	4.86502326806906\\
27.6315789473684	4.98225790991901\\
28.2894736842105	5.09949498494309\\
28.9473684210526	5.21673433019216\\
29.6052631578947	5.33397579689663\\
30.2631578947368	5.4512192489621\\
30.9210526315789	5.56846456165173\\
31.5789473684211	5.68571162042957\\
32.2368421052632	5.80296031994192\\
32.8947368421053	5.92021056311727\\
33.5526315789474	6.03746226037146\\
34.2105263157895	6.15471532890051\\
34.8684210526316	6.27196969205312\\
35.5263157894737	6.38922527877121\\
36.1842105263158	6.50648202308986\\
36.8421052631579	6.62373986369046\\
37.5	6.7409987434994\\
38.1578947368421	6.8582586093279\\
38.8157894736842	6.97551941154776\\
39.4736842105263	7.092781103799\\
40.1315789473684	7.21004364272582\\
40.7894736842105	7.32730698773674\\
41.4473684210526	7.44457110079\\
42.1052631578947	7.56183594619518\\
42.7631578947368	7.67910149043521\\
43.421052631579	7.79636770200401\\
44.0789473684211	7.91363455125764\\
44.7368421052632	8.03090201027937\\
45.3947368421053	8.1481700527556\\
46.0526315789474	8.26543865386302\\
46.7105263157895	8.38270779016425\\
47.3684210526316	8.49997743951286\\
48.0263157894737	8.61724758096587\\
48.6842105263158	8.73451819470299\\
49.3421052631579	8.85178926195305\\
50	8.96906076492473\\
50.6578947368421	9.08633268674414\\
51.3157894736842	9.20360501139643\\
51.9736842105263	9.32087772367184\\
52.6315789473684	9.43815080911588\\
53.2894736842105	9.55542425398268\\
53.9473684210526	9.67269804519267\\
54.6052631578947	9.78997217029295\\
55.2631578947368	9.90724661741864\\
55.921052631579	10.0245213752609\\
56.5789473684211	10.1417964330336\\
57.2368421052632	10.2590717804429\\
57.8947368421053	10.3763474076607\\
58.5526315789474	10.4936233052979\\
59.2105263157895	10.6108994643806\\
59.8684210526316	10.728175876327\\
60.5263157894737	10.8454525329266\\
61.1842105263158	10.96272942632\\
61.8421052631579	11.0800065489808\\
62.5	11.1972838936976\\
63.1578947368421	11.3145614535584\\
63.8157894736842	11.4318392219346\\
64.4736842105263	11.549117192467\\
65.1315789473684	11.6663953590521\\
65.7894736842105	11.7836737158295\\
};
\addlegendentry{Corollary~\ref{cor:eps}}


\end{axis}
\end{tikzpicture}%
